WERd: Using Social Text Spelling Variants for Evaluating Dialectal Speech Recognition

We study the problem of evaluating automatic speech recognition (ASR) systems that target dialectal speech input. A major challenge in this case is that the orthography of dialects is typically not standardized. From an ASR evaluation perspective, this means that there is no clear gold standard for the expected output, and several possible outputs could be considered correct according to different human annotators, which makes standard word error rate (WER) inadequate as an evaluation metric. Such a situation is typical for machine translation (MT), and thus we borrow ideas from an MT evaluation metric, namely TERp, an extension of translation error rate which is closely-related to WER. In particular, in the process of comparing a hypothesis to a reference, we make use of spelling variants for words and phrases, which we mine from Twitter in an unsupervised fashion. Our experiments with evaluating ASR output for Egyptian Arabic, and further manual analysis, show that the resulting WERd (i.e., WER for dialects) metric, a variant of TERp, is more adequate than WER for evaluating dialectal ASR.

==> baseline.tex <==
\label{sec:baselinel}
Similar to MGB2, we provide open source baseline systems for the challenge for both tasks; ASR and ADI. We also release the code for the MultiReference WER (MR-WER)\footnote{MR-WER \url{https://github.com/qcri/multiRefWER}.} as potential measure for the error rate in non-orthographic language. 

\subsection{ASR Baseline}
The baseline system uses the full MGB2 data, ie 1,200 hours. In fact, we trippled this data by applying speed and volume perturbation\cite{ko2015audio}. The recipe is available on Kaldi repository\footnote{\url{https://github.com/kaldi-asr/kaldi/tree/master/egs/gale_arabic/s5b}}. The acoustic modeling (AM) is similar to QATS submission\cite{khurana2016qcri}. The lexicon is grapheme based and covers 950K words collected from the shared lexicons as well as the training data text. The results are based on single-pass decoding using tri-gram LM along with purely sequence trained TDNN AM\cite{povey2016purely}, i-vector was used for speaker adaption. We report results for the MGB2 development data (5002 non-overlap speech segments) on which we achieve a WER of 22.6\% without LM rescoring.  This is a strong baseline compared to last year results. We report results for the MGB3 development set explained in table\ref{tab:3groups}.

Word Error Rate (WER) continues to be the most commonly used metric for evaluating  ASR. Usually, transcription of the speech signal is deterministic and one manual transcription should be a sufficient reference. However, as shown in table\ref{tab:interanno} there is at about 10\% inter-annotation disagreement across the four annotators, which is expected as dialectal Arabic lacks a standardized orthography. This year will use multi-reference WER (MR-WER)\cite{ali2015multi}. The metric simply relies on comparing the recognized text against multiple manual transcription of the speech signal, which are all considered valid references.This approach is in favor of accepting a recognized word if any of the references typed it in the same form. Table\ref{tab:ASRbaseline} shows the results for all the non-overlap speech across the four annotators (1279 speech segments).


\begin{table}[h!]
\begin{center}
\scalebox{0.75}{
\begin{tabular}{c|cccccc}
 \multicolumn{1}{c}{ } & WER1 & WER2 & WER3 & WER4 & MR-WER  \\
 \hline
 Comedy & 59.5 & 59 & 58.8  &60.4& 53.6 \\
 Cooking & 72.0 & 71.3 &  71.5 &71.2& 67.5\\
 FamilyKids & 50.2 & 48.4 & 48.3 &48.3& 43.5 \\
 Fashion & 82.2 & 81.4 & 82.0 &81.2& 78.0 \\
 Drama  & 68.8&68.5&68.8&68.2&64.5 \\
 Science & 59.3 & 57.7 & 59.5  &57.2&51.4 \\
 Sports  & 54.6 & 54.9 & 55.0  &54.4& 49.4 \\
 \hline
 \bf Overall WER & \bf 63.8& \bf 62.9 & \bf 63.3 &\bf 62.8& \bf 58.0\\
 \hline
\end{tabular}
}
 \caption{Baseline results in \% for the development data after applying surface text normalization* }
  \label{tab:ASRbaseline}
\end{center}
\end{table}

\subsection{Dialect Identification Baseline}
The baseline for the ADI task uses a multi-class support vector machine (SVM) for classification. The lexical features are obtained from a speech recognition system, and bottleneck features are generated using the i-vector framework. The overall accuracy of this baseline system for the five-classes ADI task is 57.2\%, and 60.8\% average precision and 58\% overall recall. 




==> dialectspeech.tex <==
Everything is dialectal

==> exp.tex <==
Did you do exp today?

==> intro.tex <==
The Arabic MGB3 challenge targets dialectal Arabic speech.  We call it Arabic in the Wild, as the data used comes from YouTube videos collected accross different genre. dialectal videos using YouTube channels. Following the previous MGB challenges\cite{bell2015mgb,ali2016mgb}

==> participant.tex <==
The Arabic MGB3 challenge sparked the interest of quite a number of research teams around the globe. The data has been distributed to the following teams::
\begin{enumerate}[noitemsep]
\item AALTO, Finland
\item Brno, Czech Republic
\item Cairo uni., Egypt
\item MIT, USA
\item ESAT, Belgium
\item Fitchburg, USA
\item JHU, USA
\item LORI, France
\item NDSC, China
\item QCRI, Qatar
\item RDI, Egypt
\item SESTEK, Turkey
\item Tallinn, Estonia
\item Tsinghu, China
\item UQAM, Canda
\item UTDallas, USA
\item VoiceLab, Poland
\end{enumerate}
